The Wake of a Heavy Quark in Non-Abelian Plasmas : Comparing Kinetic Theory and the AdS/CFT Correspondence

We compute the non-equilibrium stress tensor induced by a heavy quark moving through weakly coupled QCD plasma at the speed of light and compare the result to N = 4 Super Yang Mills theory at strong coupling. The QCD Boltzmann equation is reformulated as a Fokker-Planck equation in a leading log approximation which is used to compute the induced stress. The transition from nonequilibrium at short distances to equilibrium at large distances is analyzed with first and second order hydrodynamics. Even after accounting for the obvious differences in shear lengths, the strongly coupled theory is significantly better described by hydrodynamics at sub-asymptotic distances. We argue that this difference between the kinetic and AdS/CFT theories is related to the second order hydrodynamic coefficient $\tau_\pi$. $\tau_\pi$ is numerically large in units of the shear length for theories based on the Boltzmann equation.

==> HQbib.tex <==
%% Articles for ref
@article{Romatschke:2009kr,
      author         = "Romatschke, Paul",
      title          = "{Relativistic Viscous Fluid Dynamics and Non-Equilibrium
                        Entropy}",
      journal        = "Class.Quant.Grav.",
      volume         = "27",
      pages          = "025006",
      doi            = "10.1088/0264-9381/27/2/025006",
      year           = "2010",
      eprint         = "0906.4787",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "INT-PUB-09-032",
      SLACcitation   = "%%CITATION = ARXIV:0906.4787;%%",
}

@article{Betz:2010cx,
      author         = "Betz, B. and Denicol, G.S. and Koide, T. and Molnar, E.
                        and Niemi, H. and others",
      title          = "{Second order dissipative fluid dynamics from kinetic
                        theory}",
      journal        = "EPJ Web Conf.",
      volume         = "13",
      pages          = "07005",
      year           = "2011",
      eprint         = "1012.5772",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1012.5772;%%",
}

%%%  Ads Papes
@Article{Gubser:2007ga,
     author    = "Gubser, Steven S. and Pufu, Silviu S. and Yarom, Amos",
     title     = "{Sonic booms and diffusion wakes generated by a heavy quark
                  in thermal AdS/CFT}",
     journal   = "Phys. Rev. Lett.",
     volume    = "100",
     year      = "2008",
     pages     = "012301",
     eprint    = "0706.4307",
     archivePrefix = "arXiv",
     primaryClass  =  "hep-th",
     doi       = "10.1103/PhysRevLett.100.012301",
     SLACcitation  = "%%CITATION = 0706.4307;%%"
}

@article{Yarom:2007ap,
      author         = "Yarom, Amos",
      title          = "{The High momentum behavior of a quark wake}",
      journal        = "Phys.Rev.",
      volume         = "D75",
      pages          = "125010",
      doi            = "10.1103/PhysRevD.75.125010",
      year           = "2007",
      eprint         = "hep-th/0702164",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
}

@Article{Chesler:2007an,
     author    = "Chesler, Paul M. and Yaffe, Laurence G.",
     title     = "{The wake of a quark moving through a strongly-coupled
                  $\mathcal N=4$ supersymmetric Yang-Mills plasma}",
     journal   = "Phys. Rev. Lett.",
     volume    = "99",
     year      = "2007",
     pages     = "152001",
     eprint    = "0706.0368",
     archivePrefix = "arXiv",
     primaryClass  =  "hep-th",
     doi       = "10.1103/PhysRevLett.99.152001",
     SLACcitation  = "%%CITATION = 0706.0368;%%"
}

@article{CasalderreySolana:2006rq,
      author         = "Casalderrey-Solana, Jorge and Teaney, Derek",
      title          = "{Heavy quark diffusion in strongly coupled N=4
                        Yang-Mills}",
      journal        = "Phys.Rev.",
      volume         = "D74",
      pages          = "085012",
      doi            = "10.1103/PhysRevD.74.085012",
      year           = "2006",
      eprint         = "hep-ph/0605199",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
}

@article{Gubser:2006bz,
      author         = "Gubser, Steven S.",
      title          = "{Drag force in AdS/CFT}",
      journal        = "Phys.Rev.",
      volume         = "D74",
      pages          = "126005",
      doi            = "10.1103/PhysRevD.74.126005",
      year           = "2006",
      eprint         = "hep-th/0605182",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
}

@article{Kovtun:2004de,
      author         = "Kovtun, P. and Son, D.T. and Starinets, A.O.",
      title          = "{Viscosity in strongly interacting quantum field theories
                        from black hole physics}",
      journal        = "Phys.Rev.Lett.",
      volume         = "94",
      pages          = "111601",
      doi            = "10.1103/PhysRevLett.94.111601",
      year           = "2005",
      note           = "An Essay submitted to 2004 Gravity Research Foundation
                        competition",
      eprint         = "hep-th/0405231",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
}

@article{Blaizot:2003iq,
      author         = "Blaizot, J.P. and Iancu, E. and Rebhan, A.",
      title          = "{On the apparent convergence of perturbative QCD at high
                        temperature}",
      journal        = "Phys.Rev.",
      volume         = "D68",
      pages          = "025011",
      doi            = "10.1103/PhysRevD.68.025011",
      year           = "2003",
      eprint         = "hep-ph/0303045",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
}

@article{Andersen:2011ug,
      author         = "Andersen, Jens O. and Leganger, Lars E. and Strickland,
                        Michael and Su, Nan",
      title          = "{The QCD trace anomaly}",
      year           = "2011",
      note           = "* Temporary entry *",
      eprint         = "1106.0514",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
}

@article{Andersen:2011sf,
      author         = "Andersen, Jens O. and Leganger, Lars E. and Strickland,
                        Michael and Su, Nan",
      title          = "{Three-loop HTL QCD thermodynamics}",
      journal        = "JHEP",
      volume         = "1108",
      pages          = "053",
      doi            = "10.1007/JHEP08(2011)053",
      year           = "2011",
      eprint         = "1103.2528",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
}

@article{Policastro:2001yc,
      author         = "Policastro, G. and Son, D.T. and Starinets, A.O.",
      title          = "{The Shear viscosity of strongly coupled N=4
                        supersymmetric Yang-Mills plasma}",
      journal        = "Phys.Rev.Lett.",
      volume         = "87",
      pages          = "081601",
      doi            = "10.1103/PhysRevLett.87.081601",
      year           = "2001",
      eprint         = "hep-th/0104066",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
}

@article{Bhattacharyya:2008jc,
      author         = "Bhattacharyya, Sayantani and Hubeny, Veronika E and
                        Minwalla, Shiraz and Rangamani, Mukund",
      title          = "{Nonlinear Fluid Dynamics from Gravity}",
      journal        = "JHEP",
      volume         = "0802",
      pages          = "045",
      doi            = "10.1088/1126-6708/2008/02/045",
      year           = "2008",
      eprint         = "0712.2456",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
}


@article{Herzog:2006gh,
      author         = "Herzog, C.P. and Karch, A. and Kovtun, P. and Kozcaz, C.
                        and Yaffe, L.G.",
      title          = "{Energy loss of a heavy quark moving through N=4
                        supersymmetric Yang-Mills plasma}",
      journal        = "JHEP",
      volume         = "0607",
      pages          = "013",
      doi            = "10.1088/1126-6708/2006/07/013",
      year           = "2006",
      eprint         = "hep-th/0605158",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
}


@article{Chesler:2007sv,
      author         = "Chesler, Paul M. and Yaffe, Laurence G.",
      title          = "{The Stress-energy tensor of a quark moving through a
                        strongly-coupled N=4 supersymmetric Yang-Mills plasma:
                        Comparing hydrodynamics and AdS/CFT}",
      journal        = "Phys.Rev.",
      volume         = "D78",
      pages          = "045013",
      doi            = "10.1103/PhysRevD.78.045013",
      year           = "2008",
      eprint         = "0712.0050",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
}

@article{Neufeld:2008hs,
      author         = "Neufeld, R.B.",
      title          = "{Fast Partons as a Source of Energy and Momentum in a
                        Perturbative Quark-Gluon Plasma}",
      journal        = "Phys.Rev.",
      volume         = "D78",
      pages          = "085015",
      doi            = "10.1103/PhysRevD.78.085015",
      year           = "2008",
      eprint         = "0805.0385",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
}

@article{Neufeld:2008dx,
      author         = "Neufeld, R.B.",
      title          = "{Mach cones in the quark-gluon plasma: Viscosity, speed
                        of sound, and effects of finite source structure}",
      journal        = "Phys.Rev.",
      volume         = "C79",
      pages          = "054909",
      doi            = "10.1103/PhysRevC.79.054909",
      year           = "2009",
      eprint         = "0807.2996",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
}

@article{Neufeld:2009ep,
      author         = "Neufeld, R.B. and Muller, B.",
      title          = "{The sound produced by a fast parton in the quark-gluon
                        plasma is a 'crescendo'}",
      journal        = "Phys.Rev.Lett.",
      volume         = "103",
      pages          = "042301",
      doi            = "10.1103/PhysRevLett.103.042301",
      year           = "2009",
      eprint         = "0902.2950",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
}

@article{Neufeld:2011yh,
      author         = "Neufeld, R.B. and Vitev, Ivan",
      title          = "{Parton showers as sources of energy-momentum deposition
                        in the QGP and their implication for shockwave formation
                        at RHIC and at the LHC}",
      year           = "2011",
      eprint         = "1105.2067",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
}

@article{Arnold:2009ik,
      author         = "Arnold, Peter Brockway and Cantrell, Sean and Xiao, Wei",
      title          = "{Stopping distance for high energy jets in weakly-coupled
                        quark-gluon plasmas}",
      journal        = "Phys.Rev.",
      volume         = "D81",
      pages          = "045017",
      doi            = "10.1103/PhysRevD.81.045017",
      year           = "2010",
      eprint         = "0912.3862",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
}



% Experiment
@article{Adare:2008cqb,
      author         = "Adare, A. and others",
      title          = "{Dihadron azimuthal correlations in Au+Au collisions at
                        s(NN)**(1/2) = 200-GeV}",
      collaboration  = "PHENIX Collaboration",
      journal        = "Phys.Rev.",
      volume         = "C78",
      pages          = "014901",
      doi            = "10.1103/PhysRevC.78.014901",
      year           = "2008",
      eprint         = "0801.4545",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-ex",
}

@Article{Abelev:2008nda,
     author    = "Abelev, B. I. and others",
 collaboration = "STAR",
     title     = "{Indications of Conical Emission of Charged Hadrons at
                  RHIC}",
     journal   = "Phys. Rev. Lett.",
     volume    = "102",
     year      = "2009",
     pages     = "052302",
     eprint    = "0805.0622",
     archivePrefix = "arXiv",
     primaryClass  =  "nucl-ex",
     doi       = "10.1103/PhysRevLett.102.052302",
     SLACcitation  = "%%CITATION = 0805.0622;%%"
}

@Article{Chaudhuri:2005vc,
     author    = "Chaudhuri, A. K. and Heinz, Ulrich",
     title     = "{Effect of jet quenching on the hydrodynamical evolution of
                  QGP}",
     journal   = "Phys. Rev. Lett.",
     volume    = "97",
     year      = "2006",
     pages     = "062301",
     eprint    = "nucl-th/0503028",
     archivePrefix = "arXiv",
     doi       = "10.1103/PhysRevLett.97.062301",
     SLACcitation  = "%%CITATION = NUCL-TH/0503028;%%"
}


%% Older mach cone
@article{CasalderreySolana:2006sq,
      author         = "Casalderrey-Solana, J. and Shuryak, E.V. and Teaney, D.",
      title          = "{Hydrodynamic flow from fast particles}",
      year           = "2006",
      eprint         = "hep-ph/0602183",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
}

@article{CasalderreySolana:2004qm,
      author         = "Casalderrey-Solana, J. and Shuryak, E.V. and Teaney, D.",
      title          = "{Conical flow induced by quenched QCD jets}",
      journal        = "J.Phys.Conf.Ser.",
      volume         = "27",
      pages          = "22-31",
      doi            = "10.1016/j.nuclphysa.2006.06.091,
                        10.1088/1742-6596/27/1/003,
                        10.1016/j.nuclphysa.2006.06.091,
                        10.1088/1742-6596/27/1/003",
      year           = "2005",
      eprint         = "hep-ph/0411315",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
}

@article{Stoecker:2004qu,
      author         = "Stoecker, Horst",
      title          = "{Collective flow signals the quark gluon plasma}",
      journal        = "Nucl.Phys.",
      volume         = "A750",
      pages          = "121-147",
      doi            = "10.1016/j.nuclphysa.2004.12.074",
      year           = "2005",
      eprint         = "nucl-th/0406018",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
}

@article{Hong:2010at,
      author         = "Hong, Juhee and Teaney, Derek",
      title          = "{Spectral densities for hot QCD plasmas in a leading log
                        approximation}",
      journal        = "Phys.Rev.",
      volume         = "C82",
      pages          = "044908",
      doi            = "10.1103/PhysRevC.82.044908",
      year           = "2010",
      eprint         = "1003.0699",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
}

@article{Alver:2010gr,
      author         = "Alver, B. and Roland, G.",
      title          = "{Collision geometry fluctuations and triangular flow in
                        heavy-ion collisions}",
      journal        = "Phys.Rev.",
      volume         = "C81",
      pages          = "054905",
      doi            = "10.1103/PhysRevC.81.054905, 10.1103/PhysRevC.82.039903",
      year           = "2010",
      eprint         = "1003.0194",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
}

@article{Teaney:2009qa,
      author         = "Teaney, Derek A.",
      title          = "{Viscous Hydrodynamics and the Quark Gluon Plasma}",
      year           = "2009",
      eprint         = "0905.2433",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
}

@article{Baym:1990uj,
      author         = "Baym, G. and Monien, H. and Pethick, C.J. and Ravenhall, D.G.",
      title          = "{ Transverse Interactions and Transport in Relativistic Quark-Gluon and Electromagnetic Plasmas}", 
      journal        = "Phys.Rev.Lett.",
      volume         = "64",
      pages          = "1867-1870",
      doi            = "10.1103/PhysRevLett.64.1867",
      year           = "1990",
}

@article{Baier:2007ix,
      author         = "Baier, Rudolf and Romatschke, Paul and Son, Dam Thanh and
                        Starinets, Andrei O. and Stephanov, Mikhail A.",
      title          = "{Relativistic viscous hydrodynamics, conformal
                        invariance, and holography}",
      journal        = "JHEP",
      volume         = "0804",
      pages          = "100",
      doi            = "10.1088/1126-6708/2008/04/100",
      year           = "2008",
      eprint         = "0712.2451",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
}

@article{Arnold:2006fz,
      author         = "Arnold, Peter Brockway and Dogan, Caglar and Moore, Guy
                        D.",
      title          = "{The Bulk Viscosity of High-Temperature QCD}",
      journal        = "Phys.Rev.",
      volume         = "D74",
      pages          = "085021",
      doi            = "10.1103/PhysRevD.74.085021",
      year           = "2006",
      eprint         = "hep-ph/0608012",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
}

@article{Arnold:2008vd,
      author         = "Arnold, Peter Brockway and Xiao, Wei",
      title          = "{High-energy jet quenching in weakly-coupled quark-gluon
                        plasmas}",
      journal        = "Phys.Rev.",
      volume         = "D78",
      pages          = "125008",
      doi            = "10.1103/PhysRevD.78.125008",
      year           = "2008",
      eprint         = "0810.1026",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
}

@article{York:2008rr,
      author         = "York, Mark Abraao and Moore, Guy D.",
      title          = "{Second order hydrodynamic coefficients from kinetic
                        theory}",
      journal        = "Phys.Rev.",
      volume         = "D79",
      pages          = "054011",
      doi            = "10.1103/PhysRevD.79.054011",
      year           = "2009",
      eprint         = "0811.0729",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
}


@article{Arnold:2000dr,
      author         = "Arnold, Peter Brockway and Moore, Guy D. and Yaffe,
                        Laurence G.",
      title          = "{Transport coefficients in high temperature gauge
                        theories. 1. Leading log results}",
      journal        = "JHEP",
      volume         = "0011",
      pages          = "001",
      year           = "2000",
      eprint         = "hep-ph/0010177",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
}

@article{Braaten:1991we,
      author         = "Braaten, Eric and Thoma, Markus H.",
      title          = "{Energy loss of a heavy quark in the quark - gluon
                        plasma}",
      journal        = "Phys.Rev.",
      volume         = "D44",
      pages          = "2625-2630",
      doi            = "10.1103/PhysRevD.44.2625",
      year           = "1991",
}

@article{Braaten:1991jj,
      author         = "Braaten, Eric and Thoma, Markus H.",
      title          = "{Energy loss of a heavy fermion in a hot plasma}",
      journal        = "Phys.Rev.",
      volume         = "D44",
      pages          = "1298-1310",
      doi            = "10.1103/PhysRevD.44.1298",
      year           = "1991",
}


@article{Moore:2004tg,
      author         = "Moore, Guy D. and Teaney, Derek",
      title          = "{How much do heavy quarks thermalize in a heavy ion
                        collision?}",
      journal        = "Phys.Rev.",
      volume         = "C71",
      pages          = "064904",
      doi            = "10.1103/PhysRevC.71.064904",
      year           = "2005",
      eprint         = "hep-ph/0412346",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
}

@article{Israel:1979wp,
      author         = "Israel, W. and Stewart, J.M.",
      title          = "{Transient relativistic thermodynamics and kinetic
                        theory}",
      journal        = "Annals Phys.",
      volume         = "118",
      pages          = "341-372",
      doi            = "10.1016/0003-4916(79)90130-1",
      year           = "1979",
}

@article{Israel:1976tn,
      author         = "Israel, W.",
      title          = "{Nonstationary irreversible thermodynamics: A Causal
                        relativistic theory}",
      journal        = "Annals Phys.",
      volume         = "100",
      pages          = "310-331",
      doi            = "10.1016/0003-4916(76)90064-6",
      year           = "1976",
}

@article{Noronha:2008un,
      author         = "Noronha, Jorge and Gyulassy, Miklos and Torrieri,
                        Giorgio",
      title          = "{Di-Jet Conical Correlations Associated with Heavy Quark
                        Jets in anti-de Sitter Space/Conformal Field Theory
                        Correspondence}",
      journal        = "Phys.Rev.Lett.",
      volume         = "102",
      pages          = "102301",
      doi            = "10.1103/PhysRevLett.102.102301",
      year           = "2009",
      eprint         = "0807.1038",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
}

@article{Takahashi:2009na,
      author         = "Takahashi, J. and Tavares, B.M. and Qian, W.L. and
                        Andrade, R. and Grassi, F. and others",
      title          = "{Topology studies of hydrodynamics using two particle
                        correlation analysis}",
      journal        = "Phys.Rev.Lett.",
      volume         = "103",
      pages          = "242301",
      doi            = "10.1103/PhysRevLett.103.242301",
      year           = "2009",
      eprint         = "0902.4870",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
}

@article{Sorensen:2010zq,
      author         = "Sorensen, Paul",
      title          = "{Implications of space-momentum correlations and
                        geometric fluctuations in heavy-ion collisions}",
      journal        = "J.Phys.G",
      volume         = "G37",
      pages          = "094011",
      doi            = "10.1088/0954-3899/37/9/094011",
      year           = "2010",
      eprint         = "1002.4878",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-ex",
}

@article{Lin:2004en,
      author         = "Lin, Zi-Wei and Ko, Che Ming and Li, Bao-An and Zhang,
                        Bin and Pal, Subrata",
      title          = "{A Multi-phase transport model for relativistic heavy ion
                        collisions}",
      journal        = "Phys.Rev.",
      volume         = "C72",
      pages          = "064901",
      doi            = "10.1103/PhysRevC.72.064901",
      year           = "2005",
      eprint         = "nucl-th/0411110",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
}

@article{Ma:2006fm,
      author         = "Ma, G.L. and Zhang, S. and Ma, Y.G. and Huang, H.Z. and
                        Cai, X.Z. and others",
      title          = "{Di-hadron azimuthal correlation and mach-like cone
                        structure in parton/hadron transport model}",
      journal        = "Phys.Lett.",
      volume         = "B641",
      pages          = "362-367",
      doi            = "10.1016/j.physletb.2006.09.001",
      year           = "2006",
      eprint         = "nucl-th/0601012",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
}

@article{Yarom:2007ni,
      author         = "Yarom, Amos",
      title          = "{On the energy deposited by a quark moving in an N=4 SYM
                        plasma}",
      journal        = "Phys.Rev.",
      volume         = "D75",
      pages          = "105023",
      doi            = "10.1103/PhysRevD.75.105023",
      year           = "2007",
      eprint         = "hep-th/0703095",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
}

@article{Romatschke:2009kr,
      author         = "Romatschke, Paul",
      title          = "{Relativistic Viscous Fluid Dynamics and Non-Equilibrium
                        Entropy}",
      journal        = "Class.Quant.Grav.",
      volume         = "27",
      pages          = "025006",
      doi            = "10.1088/0264-9381/27/2/025006",
      year           = "2010",
      eprint         = "0906.4787",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
}

@article{Chatrchyan:2011sx,
      author         = "Chatrchyan, Serguei and others",
      title          = "{Observation and studies of jet quenching in PbPb
                        collisions at nucleon-nucleon center-of-mass energy = 2.76
                        TeV}",
      collaboration  = "CMS Collaboration",
      journal        = "Phys. Rev.",
      volume         = "C84",
      pages          = "024906",
      doi            = "10.1103/PhysRevC.84.024906",
      year           = "2011",
      eprint         = "1102.1957",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-ex",
}

@article{Maldacena:1997re,
      author         = "Maldacena, Juan Martin",
      title          = "{The Large N limit of superconformal field theories and
                        supergravity}",
      journal        = "Adv.Theor.Math.Phys.",
      volume         = "2",
      pages          = "231-252",
      doi            = "10.1023/A:1026654312961, 10.1023/A:1026654312961",
      year           = "1998",
      eprint         = "hep-th/9711200",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
}

@article{Karch:2003nh,
      author         = "Karch, A. and Katz, A.",
      title          = "{Adding flavor to AdS/CFT}",
      journal        = "Fortsch.Phys.",
      volume         = "51",
      pages          = "759-763",
      doi            = "10.1002/prop.200310094",
      year           = "2003",
}


@article{Athanasiou:2010pv,
      author         = "Athanasiou, Christiana and Chesler, Paul M. and Liu, Hong
                        and Nickel, Dominik and Rajagopal, Krishna",
      title          = "{Synchrotron radiation in strongly coupled conformal
                        field theories}",
      journal        = "Phys.Rev.",
      volume         = "D81",
      pages          = "126001",
      doi            = "10.1103/PhysRevD.81.126001",
      year           = "2010",
      eprint         = "1001.3880",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
}


@article{deHaro:2000xn,
      author         = "de Haro, Sebastian and Solodukhin, Sergey N. and
                        Skenderis, Kostas",
      title          = "{Holographic reconstruction of space-time and
                        renormalization in the AdS / CFT correspondence}",
      journal        = "Commun.Math.Phys.",
      volume         = "217",
      pages          = "595-622",
      doi            = "10.1007/s002200100381",
      year           = "2001",
      eprint         = "hep-th/0002230",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
}

@Article{Gubser:2007nd,
     author    = "Gubser, Steven S. and Pufu, Silviu S.",
     title     = "{Master field treatment of metric perturbations sourced by
                  the trailing string}",
     journal   = "Nucl. Phys.",
     volume    = "B790",
     year      = "2008",
     pages     = "42-71",
     eprint    = "hep-th/0703090",
     archivePrefix = "arXiv",
     doi       = "10.1016/j.nuclphysb.2007.08.015",
     SLACcitation  = "%%CITATION = HEP-TH/0703090;%%"
}

@article{Dominguez:2008vd,
      author         = "Dominguez, Fabio and Marquet, C. and Mueller, A.H. and
                        Wu, Bin and Xiao, Bo-Wen",
      title          = "{Comparing energy loss and p-perpendicular - broadening
                        in perturbative QCD with strong coupling N = 4 SYM
                        theory}",
      journal        = "Nucl.Phys.",
      volume         = "A811",
      pages          = "197-222",
      doi            = "10.1016/j.nuclphysa.2008.07.004",
      year           = "2008",
      eprint         = "0803.3234",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
}

@article{Gubser:2006nz,
      author         = "Gubser, Steven S.",
      title          = "{Momentum fluctuations of heavy quarks in the
                        gauge-string duality}",
      journal        = "Nucl.Phys.",
      volume         = "B790",
      pages          = "175-199",
      doi            = "10.1016/j.nuclphysb.2007.09.017",
      year           = "2008",
      eprint         = "hep-th/0612143",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
}

@article{CasalderreySolana:2007qw,
      author         = "Casalderrey-Solana, Jorge and Teaney, Derek",
      title          = "{Transverse Momentum Broadening of a Fast Quark in a N=4
                        Yang Mills Plasma}",
      journal        = "JHEP",
      volume         = "0704",
      pages          = "039",
      doi            = "10.1088/1126-6708/2007/04/039",
      year           = "2007",
      eprint         = "hep-th/0701123",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
}

@article{Hatta:2008tx,
      author         = "Hatta, Y. and Iancu, E. and Mueller, A.H.",
      title          = "{Jet evolution in the N=4 SYM plasma at strong coupling}",
      journal        = "JHEP",
      volume         = "0805",
      pages          = "037",
      doi            = "10.1088/1126-6708/2008/05/037",
      year           = "2008",
      eprint         = "0803.2481",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
}

@article{Noronha:2008un,
      author         = "Noronha, Jorge and Gyulassy, Miklos and Torrieri,
                        Giorgio",
      title          = "{Di-Jet Conical Correlations Associated with Heavy Quark
                        Jets in anti-de Sitter Space/Conformal Field Theory
                        Correspondence}",
      journal        = "Phys.Rev.Lett.",
      volume         = "102",
      pages          = "102301",
      doi            = "10.1103/PhysRevLett.102.102301",
      year           = "2009",
      eprint         = "0807.1038",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:0807.1038;%%",
}

@article{Betz:2008wy,
      author         = "Betz, Barbara and Gyulassy, Miklos and Noronha, Jorge and
                        Torrieri, Giorgio",
      title          = "{Anomalous Conical Di-jet Correlations in pQCD vs
                        AdS/CFT}",
      journal        = "Phys.Lett.",
      volume         = "B675",
      pages          = "340-346",
      doi            = "10.1016/j.physletb.2009.04.026",
      year           = "2009",
      eprint         = "0807.4526",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:0807.4526;%%",
}

@article{Noronha:2011fi,
      author         = "Noronha, Jorge and Denicol, Gabriel S.",
      title          = "{Transient Fluid Dynamics of the Quark-Gluon Plasma
                        According to AdS/CFT}",
      year           = "2011",
      eprint         = "1104.2415",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      SLACcitation   = "%%CITATION = ARXIV:1104.2415;%%",
}

@article{Denicol:2010xn,
      author         = "Denicol, G.S. and Koide, T. and Rischke, D.H.",
      title          = "{Dissipative relativistic fluid dynamics: a new way to
                        derive the equations of motion from kinetic theory}",
      journal        = "Phys.Rev.Lett.",
      volume         = "105",
      pages          = "162501",
      doi            = "10.1103/PhysRevLett.105.162501",
      year           = "2010",
      eprint         = "1004.5013",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1004.5013;%%",
}


@book{LeBellac,
 author = {M.~Le Bellac},
 title = {Thermal Field Theory},
 publisher = {Cambridge University Press},
 year = {1996}
}
 
@article{Elze:1989un,
 author = "Elze, Hans-Thomas and Heinz, Ulrich W.",
 title = "{Quark - Gluon Transport Theory}",
 journal = "Phys.Rept.",
 volume = "183",
 pages = "81-135",
 doi = "10.1016/0370-1573(89)90059-8",
 year = "1989",
 reportNumber = "CERN-TH-5325-89",
 SLACcitation = "%%CITATION = PRPLC,183,81;%%",
}
 
@article{Blaizot:2001nr,
 author = "Blaizot, Jean-Paul and Iancu, Edmond",
 title = "{The Quark gluon plasma: Collective dynamics and hard
 thermal loops}",
 journal = "Phys.Rept.",
 volume = "359",
 pages = "355-528",
 doi = "10.1016/S0370-1573(01)00061-8",
 year = "2002",
 eprint = "hep-ph/0101103",
 archivePrefix = "arXiv",
 primaryClass = "hep-ph",
 reportNumber = "SACLAY-T01-005, CERN-TH-2000-272",
 SLACcitation = "%%CITATION = HEP-PH/0101103;%%",
}
 


